Reduced sensitivity to charge noise in semiconductor spin qubits via symmetric operation

We demonstrate improved operation of exchange-coupled semiconductor quantum dots by substantially reducing the sensitivity of exchange operations to charge noise. The method involves biasing a double-dot symmetrically between the charge-state anti-crossings, where the derivative of the exchange energy with respect to gate voltages is minimized. Exchange remains highly tunable by adjusting the tunnel coupling. We find that this method reduces the dephasing effect of charge noise by more than a factor of five in comparison to operation near a charge-state anti-crossing, increasing the number of observable exchange oscillations in our qubit by a similar factor. Performance also improves with exchange rate, favoring fast quantum operations.

==> SOP_header.tex <==
% This is now the recommended way for checking for PDFLaTeX:
\RequirePackage{ifpdf}
\RequirePackage{varioref}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{color}
\RequirePackage[active]{srcltx}
%\RequirePackage{draftwatermark}
\RequirePackage{psfrag}
\RequirePackage{topcapt}
\RequirePackage{hyperref}
\RequirePackage{fancyhdr}
\RequirePackage{graphicx}
%\ifpdf
%\RequirePackage[pdftex]{graphicx}
%\else
%\RequirePackage{graphicx}
%\fi


\pagestyle{fancy}
\lhead{}
\rhead{}
\renewcommand{\headrulewidth}{0.0pt}
%\lfoot{\small\sffamily\copyright 2015 HRL Laboratories, LLC.  All Rights Reserved.}
\lfoot{\small\copyright~2015 HRL Laboratories, LLC.  All rights reserved.}
\cfoot{}
\rfoot{\thepage}

% Use utf-8 encoding for foreign characters
\usepackage[utf8]{inputenc}

% custom commands
\newcommand{\dd}[2]{\frac{{\rm d} #1}{{\rm d} #2}}
\newcommand{\pdd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ghz}{~\mathrm{GHz}}
\newcommand{\mhz}{~\mathrm{MHz}}
\newcommand{\mV}{~\mathrm{mV}}
\newcommand{\ns}{~\mathrm{ns}}
\newcommand{\neV}{~\mathrm{neV}}
\newcommand{\mK}{~\mathrm{mK}}

%\newcommand{\vx}{\widetilde{\vec{V}}_{\mathrm{X1}}} %\vec{\tilde{V}_{X1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Long comments
\long\def\comment#1{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% To save typing on all math commands
\newcommand{\mathcommand}[3][0]{\newcommand{#2}[#1]{\ensuremath{#3}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Text subscripting
\newcommand{\ts}[2]{{#1}_{\textnormal{#2}}} %A math symbol with a text subscript
\newcommand{\tsc}[2]{{#1}_{\textsc{\lowercase{#2}}}} %A math symbol with a text subscript, small caps

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Abbreviations
\newcommand{\abbrev}[1]{{\scshape\lowercase{#1}}}  % see LaTeX Companion, p. 169

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% More commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Referencing Equations
% Uses package varioref
\renewcommand{\reftextcurrent}{}
\newcommand{\refeq}[1]{Eq.~\eqref{#1}}
\newcommand{\refequation}[1]{Equation~\eqref{#1}}
\newcommand{\fullrefeq}[1]{Eq.~\eqref{#1} \vpageref{#1}}
\newcommand{\fullrefequation}[1]{Equation~\eqref{#1} \vpageref{#1}}
\newcommand{\reftwoeqs}[2]{Eqs.~\eqref{#1} and \eqref{#2}}
\newcommand{\refeqs}[1]{Eqs.~\eqref{#1}}
\newcommand{\refsec}[1]{Sec.~\ref{#1}}
\newcommand{\refexteq}[1]{Eq.~(#1)}
\newcommand{\reftable}[1]{Table~\ref{#1}}
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\refchapter}[1]{Chapter~\ref{#1}}
\newcommand{\refapp}[1]{Appendix~\ref{#1}}
\newcommand{\ibid}{\latinfont{ibid}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Hamiltonian Notation
\newcommand{\ham}[1][]{\ensuremath{{H}_{\text{#1}}}} % symbol for hamiltonian (second quantized)
\newcommand{\tildeham}[1][]{\ensuremath{{\tilde{H}}_{\text{#1}}}}
\newcommand{\hamdens}[1][]{\ensuremath{\mathcal{H}_{\text{#1}}}} %symbol for hamiltonian density
\newcommand{\tildehamdens}[1][]{\ensuremath{\tilde{\mathcal{H}}_{\text{#1}}}} %symbol for hamiltonian density with tilde
\newcommand{\barhamdens}[1][]{\ensuremath{\ts{\bar{\mathcal{H}}}{#1}}}
\mathcommand[1]{\supop}{\hat{#1}} % to promote an operator to a superoperator
\newcommand{\supham}[1][]{\ensuremath{\supop{H}_{\text{#1}}}} %symbol for hamiltonian superoperator
\mathcommand[1]{\hilbert}{\mathfrak{H}_{\text{#1}}} %symbol for Hilbert space
\newcommand{\aveham}[2][]{\bar{\mathcal{H}}^{(#2)}_{\text{#1}}} % Used for average Hamiltonian terms in paper
\mathcommand[2]{\avehamt}{\ts{\tilde{\mathcal{H}}}{#1}^{(#2)}} % Used for average Hamiltonian terms in paper
\mathcommand\hc{\text{~h.c.}}

\mathcommand{\DOS}{\mathcal{D}}  % density of states

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Bra Ket notation
\mathcommand[1]{\smallket}{|#1\rangle}
\mathcommand[1]{\smallbra}{\langle #1|}
\mathcommand[1]{\bigket}{\bigl|#1\bigr\rangle}
\mathcommand[1]{\bigbra}{\bigl\langle #1\bigr|}
\mathcommand[1]{\biggket}{\biggl|#1\biggr\rangle}
\mathcommand[1]{\biggbra}{\biggl\langle #1\biggr|}
\mathcommand[1]{\ket}{\left| #1 \right\rangle}  %a Ket
\mathcommand[1]{\lket}{\bigl| #1 \bigr)}  %a Liouville Ket
\mathcommand[1]{\bra}{\left\langle #1 \right|}  %a Bra
\mathcommand[1]{\lbra}{\bigl( #1 \bigr|}  %a Bra
\newcommand{\ketbra}[2]{\left| #1 \right\rangle\!\!\left\langle #2
\right|} %an outer product
\newcommand{\braket}[2]{\left\langle #1 |#2\right\rangle} %an inner product
\newcommand{\bigbraket}[2]{\bigl\langle #1 \bigl| #2 \bigr\rangle} %an inner product
\newcommand{\biggbraket}[2]{\biggl\langle #1 \biggl| #2 \biggr\rangle} %an inner product
\newcommand{\bigketbra}[2]{\bigl| #1 \bigr\rangle\!\bigl\langle #2
\bigr|} %an outer product
\newcommand{\lbraket}[2]{\bigl( #1 \bigl| #2 \bigr)} %an inner product
\newcommand{\lketbra}[2]{\bigl| #1 \bigr)\!\!\bigl( #2
\bigr|} %an outer product
\newcommand{\sizedlbraket}[2]{\left.\left( #1 \left| #2 \right)\right.\right.} %an inner product
\newcommand{\biglbraket}[2]{\biggl(#1\biggl|#2\biggr)}
    % This one (above) scales to the right size, but:
    % works only if bra is smaller than ket
    % If something else is needed, define \rbraket
    % These Always make big delimiters
\newcommand{\bbraket}[2]{\biggl\langle #1 \biggm| #2 \biggr\rangle}
\mathcommand[1]{\bbra}{\biggl\langle #1 \biggr|}
\mathcommand[1]{\bket}{\biggl| #1 \biggr\rangle}
\newcommand{\gsket}{\ket{\Omega}}  %Ground state
\newcommand{\gsbra}{\bra{\Omega}}

\mathcommand{\upket}{\ket{\uparrow}}
\mathcommand{\downket}{\ket{\downarrow}}
\mathcommand{\upbra}{\bra{\uparrow}}
\mathcommand{\downbra}{\bra{\downarrow}}
\mathcommand{\upupket}{\ket{\uparrow\uparrow}}
\mathcommand{\updownket}{\ket{\uparrow\downarrow}}
\mathcommand{\downupket}{\ket{\downarrow\uparrow}}
\mathcommand{\downdownket}{\ket{\downarrow\downarrow}}

\mathcommand{\cnot}{\text{c-}\textsc{not}}
\mathcommand{\cZ}{\text{c-}Z}

%%%%%%%%%%%%%%%%%%%%%%%%% Phantom commands
\newcommand{\nodag}{{\phantom{\dag}}} %use c^\nodag to space it like c^\dag
\newcommand{\nostar}{{\phantom{*}}} % not sure if this will work

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Trace
\newcommand{\Tr}[2][]{\text{Tr}_\text{#1}\left\{#2\right\}}

%%%%%%%%%%%%%%%%% Some common vectors
\renewcommand{\vec}[1]{\ensuremath{\text{\textbf{#1}}}} % Simply a bold charactor.
    % Boldsymbol in addition to \mathbf works for Greek letters

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Equation Environments
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\splitstart}{\begin{equation}\begin{split}}
\newcommand{\splitstop}{\end{split}\end{equation}} %Why doesn't this work?!?

%%%%%%%%%%%%%%%%%%% Miscellaneous
\mathcommand{\infinity}{\infty}
\renewcommand{\Im}[1]{\ensuremath{
    \text{Im}\left\{#1\right\}}}
\renewcommand{\Re}[1]{\ensuremath{
    \text{Re}\left\{#1\right\}}}
\mathcommand{\dftnorm}{\frac{1}{\sqrt{N}}}
\mathcommand{\onehalf}{\frac{1}{2}}
\mathcommand[1]{\nth}{#1^{\text{th}}}
\mathcommand[4]{\columnvector}{\left(\begin{array}{c}
            #1\\#2\\#3\\#4 \end{array}\right)}
\mathcommand[4]{\specfunc}{#1_{#2}^{#3}\!\!\left(#4\right)} %For example, spherical harmonic, Laguerre polynomials
\newcommand{\partialby}[1]{\frac{\partial}{\partial{#1}}}
\newcommand{\sqpartialby}[1]{\frac{\partial^2}{\partial{#1}^2}}
\newcommand{\dbyd}[1]{\frac{d}{d#1}}
\mathcommand{\radtwo}{\sqrt{2}}
\mathcommand[1]{\oneover}{\frac{1}{#1}}
\newcommand{\mymatrix}[1]{\left(\begin{array}{ccc} #1
\end{array}\right)}
\newcommand{\rmatrix}[1]{\left(\begin{array}{rrr} #1
\end{array}\right)}
\mathcommand[1]{\specialsum}{{\sum_{#1}}^*}

%%%%%%%%%%%%%%%%%%%%% functions
\mathcommand{\erf}{{\rm erf}}
\mathcommand{\erfc}{{\rm erfc}}
\mathcommand{\sech}{{\rm sech}}
\mathcommand{\csch}{{\rm csch}}
\newcommand{\sinc}[1][]{\ensuremath{{\rm sinc}_{#1}}}
\mathcommand[1]{\floor}{\left\lfloor #1 \right\rfloor}
\mathcommand[1]{\ceil}{\left\lceil #1 \right\rceil}

%%%%%%%%%%%%%%%%%%% Struts
\newcommand{\mystrut}{\rule{0pt}{2.3ex}} % An x is the height of the LC letter x
\newcommand{\tablestrut}{\rule{0ex}{2.6ex}} % Gratzer, p. 151

%%%%%%%%%%%%%%%%%%% See p. 108, LaTeX Companion
\newcommand{\PBS}[1]{\let\temp=\\ #1 \let\\=\temp}
\newcommand{\narrowcol}{\PBS\raggedright\hspace{0pt}}

%%%%%%%%%%%%%%%%%%%%%%% Latin
\newcommand{\latinfont}[1]{#1}  % I think this is what the Chi. Man. of Style suggests
%\newcommand{\latinfont}[1]{\textit{#1}}
\newcommand{\ie}{\latinfont{i.e.}}
\newcommand{\via}{\latinfont{via}}
\newcommand{\eg}{\latinfont{e.g.}}
\newcommand{\cf}{\latinfont{cf.}}
\newcommand{\etal}{\latinfont{et al.}} %Note period is omitted to be used in BibTeX
\newcommand{\vs}{\latinfont{vs.}}
% I don't know how to change the et al. used by BibTeX, and it is not italic.
% kluge solution:
\newcommand{\bibetal}[2]{{#1 #2 \etal}}

%%%%%%%%%%%%%%%%%%%%%%% Temp fig
\newcommand{\tempfig}[4]{
    \begin{figure}
    \centering
    \boxed{
    \makebox[#1][c]{
    \begin{tabular}{c}
    \rule{0pt}{#2} \\
    \Huge #3 \\
    \rule{0pt}{#2}\\
    \end{tabular}}}
    \caption{#4 \label{#3}}
    \end{figure}}

% Some common colors
\newcommand{\green}{\textcolor[rgb]{0,0.4,0}}
\newcommand{\purple}{\textcolor[rgb]{0.8,0.2,0.6}} %Chosen to match standard Powerpoint colors
\newcommand{\blue}{\textcolor[rgb]{0,0,0.7}}
\newcommand{\red}{\textcolor{red}}
\newcommand{\teal}{\textcolor[rgb]{0,0.4,0.3}}
\newcommand{\darkyellow}{\textcolor[rgb]{0.8,0.6,0}}
\newcommand{\orange}{\textcolor[rgb]{1,0.4,0}}

% dense lists
\newenvironment{denseitemize}
    {\begin{list}{$\bullet$}{%
        \setlength{\topsep}{0in}
        \setlength{\parsep}{0in}
        \setlength{\itemsep}{0in}
        \setlength{\labelwidth}{3ex}
        \setlength{\leftmargin}{\labelwidth}
        \setlength{\rightmargin}{0in}
        }%
    }%
{\end{list}}

\newenvironment{densesubitemize}
    {\begin{list}{$-$}{%
        \setlength{\topsep}{0in}
        \setlength{\parsep}{0in}
        \setlength{\itemsep}{0in}
        \setlength{\rightmargin}{0in}
        }%
    }%
{\end{list}}

\newcounter{denseenumeratecounter}
\newlength{\denseenumeratelabel}
\settowidth{\denseenumeratelabel}{99.\hfil}
\newenvironment{denseenumerate}
    {\setcounter{denseenumeratecounter}{0}
        \begin{list}{\arabic{enumi}}{%
        \setlength{\topsep}{0in}
        \setlength{\parsep}{0in}
        \setlength{\itemsep}{0in}
        \setlength{\labelwidth}{\denseenumeratelabel}
        \setlength{\leftmargin}{\labelwidth}
        \addtolength{\leftmargin}{3pt}
        \setlength{\rightmargin}{0in}
        \renewcommand{\makelabel}[1]{%
            \stepcounter{denseenumeratecounter}
            \arabic{denseenumeratecounter}.\hfil}
        }%
    }%
{\end{list}}
\newcommand\Ci{\text{Ci}}
\mathcommand{\ta}{\boldsymbol\tau}
\mathcommand{\ev}{\boldsymbol\epsilon}
\mathcommand[1]{\cvec}{\overline{#1}}
\mathcommand{\trmat}{\cvec{\text{Tr}}}

\mathcommand\tc{\ts{t}{c}}


\mathcommand\tO{\ts{t}{O}}
\mathcommand\tE{\ts{t}{E}}
\mathcommand{\Sket}{\ts{\ket{S}}{O}}
\newcommand{\Optical}[1]{\ts{#1}{O}}
\mathcommand{\Tket}{\Optical{\ket{T_0}}}
\mathcommand{\Tbra}{\bra{T_0}}
\mathcommand\JO{\Optical{J}}
\mathcommand\JE{\ts{J}{E}}
\mathcommand\JOE{\ts{J}{OE}}
\mathcommand\vac{\ket{\text{vac}}}
\mathcommand\tCZ{\ts{t}{CZ}}

\newcommand{\frontmatter}[1]{%\date\today

\ifpdf
\DeclareGraphicsExtensions{.pdf, .jpg, .tif}
\else
\DeclareGraphicsExtensions{.eps, .jpg}
\fi

\begin{abstract}
	#1
\end{abstract}

\maketitle
\thispagestyle{fancy}
}

